Privacy-preserving design of graph neural networks with applications to vertical federated learning

The paradigm of vertical federated learning (VFL), where institutions collaboratively train machine learning models via combining each other's local feature or label information, has achieved great success in applications to financial risk management (FRM). The surging developments of graph representation learning (GRL) have opened up new opportunities for FRM applications under FL via efficiently utilizing the graph-structured data generated from underlying transaction networks. Meanwhile, transaction information is often considered highly sensitive. To prevent data leakage during training, it is critical to develop FL protocols with formal privacy guarantees. In this paper, we present an end-to-end GRL framework in the VFL setting called VESPER, which is built upon a general privatization scheme termed perturbed message passing (PMP) that allows the privatization of many popular graph neural architectures.Based on PMP, we discuss the strengths and weaknesses of specific design choices of concrete graph neural architectures and provide solutions and improvements for both dense and sparse graphs. Extensive empirical evaluations over both public datasets and an industry dataset demonstrate that VESPER is capable of training high-performance GNN models over both sparse and dense graphs under reasonable privacy budgets.

==> figures/ablation/batch_size/alipay/gcn_c_small.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=lightgray204
},
scale only axis,
width=2.25cm,
height=2cm,
tick align=outside,
tick pos=left,
title={Finance},
tick label style={font=\tiny},
title style={yshift=-4pt},
xticklabel style={yshift=2pt},
yticklabel style={xshift=2pt},
legend style={nodes={scale=0.5, transform shape}},
% major tick length=\MajorTickLength,
every tick/.style={
black,
semithick,
},
x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\tiny},
y label style={at={(axis description cs:-0.12,.5)},rotate=90,anchor=south,font=\tiny},
x grid style={darkgray176},
xlabel={$\epsilon$},
xmin=2.6, xmax=33.4,
xtick style={color=black},
y grid style={darkgray176},
ylabel={AUC},
ymin=0.61243575817462, ymax=0.74161759415126,
ytick style={color=black}
]
\path [fill=steelblue31119180, fill opacity=0.2]
(axis cs:4,0.713308700130452)
--(axis cs:4,0.695578977852054)
--(axis cs:8,0.704781784510618)
--(axis cs:16,0.719910308412774)
--(axis cs:32,0.714425147422215)
--(axis cs:32,0.734565121769204)
--(axis cs:32,0.734565121769204)
--(axis cs:16,0.731320865663228)
--(axis cs:8,0.723067670314412)
--(axis cs:4,0.713308700130452)
--cycle;

\path [fill=darkorange25512714, fill opacity=0.2]
(axis cs:4,0.70839626709129)
--(axis cs:4,0.692277979516865)
--(axis cs:8,0.699571530682937)
--(axis cs:16,0.715609827336004)
--(axis cs:32,0.71606570449207)
--(axis cs:32,0.738418775136088)
--(axis cs:32,0.738418775136088)
--(axis cs:16,0.729969284859488)
--(axis cs:8,0.72079289255505)
--(axis cs:4,0.70839626709129)
--cycle;

\path [fill=forestgreen4416044, fill opacity=0.2]
(axis cs:4,0.703227460751436)
--(axis cs:4,0.691804671974662)
--(axis cs:8,0.706913427000345)
--(axis cs:16,0.712626840839856)
--(axis cs:32,0.715895241392506)
--(axis cs:32,0.732725447795712)
--(axis cs:32,0.732725447795712)
--(axis cs:16,0.719248321473524)
--(axis cs:8,0.716053740701018)
--(axis cs:4,0.703227460751436)
--cycle;

\path [fill=crimson2143940, fill opacity=0.2]
(axis cs:4,0.704972425085373)
--(axis cs:4,0.688589781134879)
--(axis cs:8,0.697322619439467)
--(axis cs:16,0.703224600469374)
--(axis cs:32,0.705890440995683)
--(axis cs:32,0.7233400179115)
--(axis cs:32,0.7233400179115)
--(axis cs:16,0.71891231794628)
--(axis cs:8,0.706531200887055)
--(axis cs:4,0.704972425085373)
--cycle;

\path [fill=mediumpurple148103189, fill opacity=0.2]
(axis cs:4,0.690803028415663)
--(axis cs:4,0.674442394832635)
--(axis cs:8,0.693636163542217)
--(axis cs:16,0.691108045632734)
--(axis cs:32,0.70313692115139)
--(axis cs:32,0.718512128816626)
--(axis cs:32,0.718512128816626)
--(axis cs:16,0.710183066067861)
--(axis cs:8,0.700547265202993)
--(axis cs:4,0.690803028415663)
--cycle;

\addplot [semithick, steelblue31119180]
table {%
4 0.704443838991253
8 0.713924727412515
16 0.725615587038001
32 0.724495134595709
};
\addlegendentry{$B=32$}
\addplot [semithick, darkorange25512714]
table {%
4 0.700337123304077
8 0.710182211618993
16 0.722789556097746
32 0.727242239814079
};
\addlegendentry{$B=64$}
\addplot [semithick, forestgreen4416044]
table {%
4 0.697516066363049
8 0.711483583850682
16 0.71593758115669
32 0.724310344594109
};
\addlegendentry{$B=128$}
\addplot [semithick, crimson2143940]
table {%
4 0.696781103110126
8 0.701926910163261
16 0.711068459207827
32 0.714615229453592
};
\addlegendentry{$B=256$}
\addplot [semithick, mediumpurple148103189]
table {%
4 0.682622711624149
8 0.697091714372605
16 0.700645555850297
32 0.710824524984008
};
\addlegendentry{$B=512$}
\end{axis}

\end{tikzpicture}


==> figures/ablation/batch_size/ogb/gcn_c_small.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=lightgray204
},
scale only axis,
width=2.25cm,
height=2cm,
tick align=outside,
tick pos=left,
title={\ogb},
title style={yshift=-4pt},
xticklabel style={yshift=2pt},
yticklabel style={xshift=2pt},
tick label style={font=\tiny},
legend style={nodes={scale=0.5, transform shape}},
% major tick length=\MajorTickLength,
every tick/.style={
black,
semithick,
},
x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\tiny},
y label style={at={(axis description cs:-0.12,.5)},rotate=90,anchor=south,font=\tiny},
x grid style={darkgray176},
xlabel={$\epsilon$},
xmin=2.6, xmax=33.4,
xtick style={color=black},
y grid style={darkgray176},
ylabel={ACC},
ymin=0.550021201868666, ymax=0.715001968479474,
ytick style={color=black}
]
\path [fill=steelblue31119180, fill opacity=0.2]
(axis cs:4,0.671236894707091)
--(axis cs:4,0.663300004137105)
--(axis cs:8,0.667405408960443)
--(axis cs:16,0.69588391704559)
--(axis cs:32,0.700655316445865)
--(axis cs:32,0.708866479088074)
--(axis cs:32,0.708866479088074)
--(axis cs:16,0.706809600753723)
--(axis cs:8,0.683173306510362)
--(axis cs:4,0.671236894707091)
--cycle;

\path [fill=darkorange25512714, fill opacity=0.2]
(axis cs:4,0.66886731322877)
--(axis cs:4,0.660745703136125)
--(axis cs:8,0.667408222492391)
--(axis cs:16,0.693269748060835)
--(axis cs:32,0.696276638146028)
--(axis cs:32,0.708335915065746)
--(axis cs:32,0.708335915065746)
--(axis cs:16,0.701005317898947)
--(axis cs:8,0.674953930713239)
--(axis cs:4,0.66886731322877)
--cycle;

\path [fill=forestgreen4416044, fill opacity=0.2]
(axis cs:4,0.661566064851102)
--(axis cs:4,0.654723233691073)
--(axis cs:8,0.659735830694155)
--(axis cs:16,0.683382755017522)
--(axis cs:32,0.692330753403105)
--(axis cs:32,0.698832465822855)
--(axis cs:32,0.698832465822855)
--(axis cs:16,0.693241974828652)
--(axis cs:8,0.671167869153705)
--(axis cs:4,0.661566064851102)
--cycle;

\path [fill=crimson2143940, fill opacity=0.2]
(axis cs:4,0.640790701080829)
--(axis cs:4,0.632549617957114)
--(axis cs:8,0.655358106646228)
--(axis cs:16,0.67075906416104)
--(axis cs:32,0.684257186253877)
--(axis cs:32,0.692208218919249)
--(axis cs:32,0.692208218919249)
--(axis cs:16,0.684075418469814)
--(axis cs:8,0.664433442820106)
--(axis cs:4,0.640790701080829)
--cycle;

\path [fill=mediumpurple148103189, fill opacity=0.2]
(axis cs:4,0.589910447416111)
--(axis cs:4,0.586156691260066)
--(axis cs:8,0.631834954046615)
--(axis cs:16,0.648690737769499)
--(axis cs:32,0.664850410998202)
--(axis cs:32,0.675176727515307)
--(axis cs:32,0.675176727515307)
--(axis cs:16,0.660078128942263)
--(axis cs:8,0.64793953331066)
--(axis cs:4,0.589910447416111)
--cycle;

\addplot [semithick, steelblue31119180]
table {%
4 0.667268449422098
8 0.675289357735403
16 0.701346758899657
32 0.704760897766969
};
\addlegendentry{$B=32$}
\addplot [semithick, darkorange25512714]
table {%
4 0.664806508182447
8 0.671181076602815
16 0.697137532979891
32 0.702306276605887
};
\addlegendentry{$B=64$}
\addplot [semithick, forestgreen4416044]
table {%
4 0.658144649271087
8 0.66545184992393
16 0.688312364923087
32 0.69558160961298
};
\addlegendentry{$B=128$}
\addplot [semithick, crimson2143940]
table {%
4 0.636670159518972
8 0.659895774733167
16 0.677417241315427
32 0.688232702586563
};
\addlegendentry{$B=256$}
\addplot [semithick, mediumpurple148103189]
table {%
4 0.588033569338089
8 0.639887243678638
16 0.654384433355881
32 0.670013569256754
};
\addlegendentry{$B=512$}
\end{axis}

\end{tikzpicture}


==> figures/ablation/batch_size/reddit/gcn_c_small.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=lightgray204
},
scale only axis,
width=2.25cm,
height=2cm,
tick align=outside,
tick pos=left,
title={Reddit},
title style={yshift=-4pt},
xticklabel style={yshift=2pt},
yticklabel style={xshift=2pt},
tick label style={font=\tiny},
legend style={nodes={scale=0.5, transform shape}},
% major tick length=\MajorTickLength,
every tick/.style={
black,
semithick,
},
x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\tiny},
y label style={at={(axis description cs:-0.12,.5)},rotate=90,anchor=south,font=\tiny},
x grid style={darkgray176},
xlabel={$\epsilon$},
xmin=2.6, xmax=33.4,
xtick style={color=black},
y grid style={darkgray176},
ylabel={ACC},
ymin=0.784170537257303, ymax=0.933870273368051,
ytick style={color=black}
]
\path [fill=steelblue31119180, fill opacity=0.2]
(axis cs:4,0.901205130589604)
--(axis cs:4,0.895829140455044)
--(axis cs:8,0.91111645676936)
--(axis cs:16,0.919163365854363)
--(axis cs:32,0.924299536647549)
--(axis cs:32,0.927065739908471)
--(axis cs:32,0.927065739908471)
--(axis cs:16,0.923085705111293)
--(axis cs:8,0.914465648323723)
--(axis cs:4,0.901205130589604)
--cycle;

\path [fill=darkorange25512714, fill opacity=0.2]
(axis cs:4,0.892838702927744)
--(axis cs:4,0.88907968566892)
--(axis cs:8,0.905409162413522)
--(axis cs:16,0.913719884370103)
--(axis cs:32,0.9225875670483)
--(axis cs:32,0.92542061922533)
--(axis cs:32,0.92542061922533)
--(axis cs:16,0.917201250936792)
--(axis cs:8,0.909013759152642)
--(axis cs:4,0.892838702927744)
--cycle;

\path [fill=forestgreen4416044, fill opacity=0.2]
(axis cs:4,0.883220509824135)
--(axis cs:4,0.877664900297402)
--(axis cs:8,0.893884424443282)
--(axis cs:16,0.909764709167118)
--(axis cs:32,0.915235970241586)
--(axis cs:32,0.918442646709027)
--(axis cs:32,0.918442646709027)
--(axis cs:16,0.912503391294257)
--(axis cs:8,0.897433816944076)
--(axis cs:4,0.883220509824135)
--cycle;

\path [fill=crimson2143940, fill opacity=0.2]
(axis cs:4,0.866485105222174)
--(axis cs:4,0.860976611381959)
--(axis cs:8,0.884583529905576)
--(axis cs:16,0.897946393650631)
--(axis cs:32,0.911471687134752)
--(axis cs:32,0.913877037350464)
--(axis cs:32,0.913877037350464)
--(axis cs:16,0.904369460073585)
--(axis cs:8,0.887579549282259)
--(axis cs:4,0.866485105222174)
--cycle;

\path [fill=mediumpurple148103189, fill opacity=0.2]
(axis cs:4,0.821573625044567)
--(axis cs:4,0.790975070716882)
--(axis cs:8,0.86750988794471)
--(axis cs:16,0.886009058274813)
--(axis cs:32,0.89948394198981)
--(axis cs:32,0.904451214105913)
--(axis cs:32,0.904451214105913)
--(axis cs:16,0.888810969371813)
--(axis cs:8,0.87651826134707)
--(axis cs:4,0.821573625044567)
--cycle;

\addplot [semithick, steelblue31119180]
table {%
4 0.898517135522324
8 0.912791052546541
16 0.921124535482828
32 0.92568263827801
};
\addlegendentry{$B=32$}
\addplot [semithick, darkorange25512714]
table {%
4 0.890959194298332
8 0.907211460783082
16 0.915460567653448
32 0.924004093136815
};
\addlegendentry{$B=64$}
\addplot [semithick, forestgreen4416044]
table {%
4 0.880442705060769
8 0.895659120693679
16 0.911134050230688
32 0.916839308475306
};
\addlegendentry{$B=128$}
\addplot [semithick, crimson2143940]
table {%
4 0.863730858302066
8 0.886081539593918
16 0.901157926862108
32 0.912674362242608
};
\addlegendentry{$B=256$}
\addplot [semithick, mediumpurple148103189]
table {%
4 0.806274347880725
8 0.87201407464589
16 0.887410013823313
32 0.901967578047861
};
\addlegendentry{$B=512$}
\end{axis}

\end{tikzpicture}


==> figures/ablation/max_degree/alipay/gcn_c_small.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=lightgray204
},
scale only axis,
width=2.25cm,
height=2cm,
tick align=outside,
tick pos=left,
title={Finance},
title style={yshift=-4pt},
xticklabel style={yshift=2pt},
yticklabel style={xshift=2pt},
tick label style={font=\tiny},
legend style={nodes={scale=0.5, transform shape}},
% major tick length=\MajorTickLength,
every tick/.style={
black,
semithick,
},
x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\tiny},
y label style={at={(axis description cs:-0.12,.5)},rotate=90,anchor=south,font=\tiny},
x grid style={darkgray176},
xlabel={$\epsilon$},
xmin=2.6, xmax=33.4,
xtick style={color=black},
y grid style={darkgray176},
ylabel={AUC},
ymin=0.692762525649503, ymax=0.740592882254496,
ytick style={color=black}
]
\path [fill=steelblue31119180, fill opacity=0.2]
(axis cs:4,0.713308700130452)
--(axis cs:4,0.695578977852054)
--(axis cs:8,0.704781784510618)
--(axis cs:16,0.719910308412774)
--(axis cs:32,0.71606570449207)
--(axis cs:32,0.738418775136088)
--(axis cs:32,0.738418775136088)
--(axis cs:16,0.731320865663228)
--(axis cs:8,0.723067670314412)
--(axis cs:4,0.713308700130452)
--cycle;

\path [fill=darkorange25512714, fill opacity=0.2]
(axis cs:4,0.709416774789518)
--(axis cs:4,0.694936632767912)
--(axis cs:8,0.705384348211806)
--(axis cs:16,0.712760467484455)
--(axis cs:32,0.71376828584445)
--(axis cs:32,0.730895476197186)
--(axis cs:32,0.730895476197186)
--(axis cs:16,0.724262924768823)
--(axis cs:8,0.717196366459426)
--(axis cs:4,0.709416774789518)
--cycle;

\addplot [semithick, steelblue31119180]
table {%
4 0.704443838991253
8 0.713924727412515
16 0.725615587038001
32 0.727242239814079
};
\addlegendentry{$D=10$}
\addplot [semithick, darkorange25512714]
table {%
4 0.702176703778715
8 0.711290357335616
16 0.718511696126639
32 0.722331881020818
};
\addlegendentry{$D=20$}
\end{axis}

\end{tikzpicture}


==> figures/ablation/max_degree/ogb/gcn_c_small.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=lightgray204
},
scale only axis,
width=2.25cm,
height=2cm,
tick align=outside,
tick pos=left,
title={\ogb},
tick label style={font=\tiny},
title style={yshift=-4pt},
xticklabel style={yshift=2pt},
yticklabel style={xshift=2pt},
legend style={nodes={scale=0.5, transform shape}},
% major tick length=\MajorTickLength,
every tick/.style={
black,
semithick,
},
x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\tiny},
y label style={at={(axis description cs:-0.12,.5)},rotate=90,anchor=south,font=\tiny},
x grid style={darkgray176},
xlabel={$\epsilon$},
xmin=2.6, xmax=33.4,
xtick style={color=black},
y grid style={darkgray176},
ylabel={ACC},
ymin=0.66081423309623, ymax=0.712373938231697,
ytick style={color=black}
]
\path [fill=steelblue31119180, fill opacity=0.2]
(axis cs:4,0.671236894707091)
--(axis cs:4,0.663300004137105)
--(axis cs:8,0.669329899195047)
--(axis cs:16,0.69588391704559)
--(axis cs:32,0.700655316445865)
--(axis cs:32,0.708866479088074)
--(axis cs:32,0.708866479088074)
--(axis cs:16,0.706809600753723)
--(axis cs:8,0.679990937589342)
--(axis cs:4,0.671236894707091)
--cycle;

\path [fill=darkorange25512714, fill opacity=0.2]
(axis cs:4,0.671150584038842)
--(axis cs:4,0.663157856056933)
--(axis cs:8,0.667405408960443)
--(axis cs:16,0.693967663977903)
--(axis cs:32,0.693855561992977)
--(axis cs:32,0.710030315270994)
--(axis cs:32,0.710030315270994)
--(axis cs:16,0.707777587347054)
--(axis cs:8,0.683173306510362)
--(axis cs:4,0.671150584038842)
--cycle;

\addplot [semithick, steelblue31119180]
table {%
4 0.667268449422098
8 0.674660418392194
16 0.701346758899657
32 0.704760897766969
};
\addlegendentry{$D=20$}
\addplot [semithick, darkorange25512714]
table {%
4 0.667154220047888
8 0.675289357735403
16 0.700872625662478
32 0.701942938631986
};
\addlegendentry{$D=50$}
\end{axis}

\end{tikzpicture}


==> figures/ablation/max_degree/reddit/gcn_c_small.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=lightgray204
},
scale only axis,
width=2.25cm,
height=2cm,
tick align=outside,
tick pos=left,
title={Reddit},
title style={yshift=-4pt},
xticklabel style={yshift=2pt},
yticklabel style={xshift=2pt},
tick label style={font=\tiny},
legend style={nodes={scale=0.5, transform shape}},
% major tick length=\MajorTickLength,
every tick/.style={
black,
semithick,
},
x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\tiny},
y label style={at={(axis description cs:-0.12,.5)},rotate=90,anchor=south,font=\tiny},
x grid style={darkgray176},
xlabel={$\epsilon$},
xmin=2.6, xmax=33.4,
xtick style={color=black},
y grid style={darkgray176},
ylabel={ACC},
ymin=0.889446033417524, ymax=0.928857154503278,
ytick style={color=black}
]
\path [fill=steelblue31119180, fill opacity=0.2]
(axis cs:4,0.901205130589604)
--(axis cs:4,0.895829140455044)
--(axis cs:8,0.900666337896145)
--(axis cs:16,0.908276333396107)
--(axis cs:32,0.909589798806771)
--(axis cs:32,0.915916906397616)
--(axis cs:32,0.915916906397616)
--(axis cs:16,0.913521415378645)
--(axis cs:8,0.907627649860349)
--(axis cs:4,0.901205130589604)
--cycle;

\path [fill=darkorange25512714, fill opacity=0.2]
(axis cs:4,0.901179477467445)
--(axis cs:4,0.891237448012331)
--(axis cs:8,0.91111645676936)
--(axis cs:16,0.919163365854363)
--(axis cs:32,0.924299536647549)
--(axis cs:32,0.927065739908471)
--(axis cs:32,0.927065739908471)
--(axis cs:16,0.923085705111293)
--(axis cs:8,0.914465648323723)
--(axis cs:4,0.901179477467445)
--cycle;

\addplot [semithick, steelblue31119180]
table {%
4 0.898517135522324
8 0.904146993878247
16 0.910898874387376
32 0.912753352602194
};
\addlegendentry{$D=20$}
\addplot [semithick, darkorange25512714]
table {%
4 0.896208462739888
8 0.912791052546541
16 0.921124535482828
32 0.92568263827801
};
\addlegendentry{$D=50$}
\end{axis}

\end{tikzpicture}


==> figures/ablation/min_degree/alipay/gcn_c_small.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=lightgray204
},
scale only axis,
width=2.25cm,
height=2cm,
tick align=outside,
tick pos=left,
title={Finance},
tick label style={font=\tiny},
title style={yshift=-4pt},
xticklabel style={yshift=2pt},
yticklabel style={xshift=2pt},
legend style={nodes={scale=0.5, transform shape}},
% major tick length=\MajorTickLength,
every tick/.style={
black,
semithick,
},
x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\tiny},
y label style={at={(axis description cs:-0.12,.5)},rotate=90,anchor=south,font=\tiny},
x grid style={darkgray176},
xlabel={$\epsilon$},
xmin=2.6, xmax=33.4,
xtick style={color=black},
y grid style={darkgray176},
ylabel={AUC},
ymin=0.643220052924958, ymax=0.742952047622332,
ytick style={color=black}
]
\path [fill=steelblue31119180, fill opacity=0.2]
(axis cs:4,0.713308700130452)
--(axis cs:4,0.695578977852054)
--(axis cs:8,0.704781784510618)
--(axis cs:16,0.719910308412774)
--(axis cs:32,0.71606570449207)
--(axis cs:32,0.738418775136088)
--(axis cs:32,0.738418775136088)
--(axis cs:16,0.731320865663228)
--(axis cs:8,0.723067670314412)
--(axis cs:4,0.713308700130452)
--cycle;

\path [fill=darkorange25512714, fill opacity=0.2]
(axis cs:4,0.687253964588904)
--(axis cs:4,0.647753325411202)
--(axis cs:8,0.669942860732738)
--(axis cs:16,0.67852723481068)
--(axis cs:32,0.681161788642319)
--(axis cs:32,0.702097030521673)
--(axis cs:32,0.702097030521673)
--(axis cs:16,0.689658895135507)
--(axis cs:8,0.694249024278113)
--(axis cs:4,0.687253964588904)
--cycle;

\addplot [semithick, steelblue31119180]
table {%
4 0.704443838991253
8 0.713924727412515
16 0.725615587038001
32 0.727242239814079
};
\addlegendentry{$\mind=3$}
\addplot [semithick, darkorange25512714]
table {%
4 0.667503645000053
8 0.682095942505425
16 0.684093064973094
32 0.691629409581996
};
\addlegendentry{$\mind=5$}
\end{axis}

\end{tikzpicture}


==> figures/ablation/min_degree/ogb/gcn_c_small.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=lightgray204
},
scale only axis,
width=2.25cm,
height=2cm,
tick align=outside,
tick pos=left,
title={\ogb},
title style={yshift=-4pt},
xticklabel style={yshift=2pt},
yticklabel style={xshift=2pt},
tick label style={font=\tiny},
legend style={nodes={scale=0.5, transform shape}},
% major tick length=\MajorTickLength,
every tick/.style={
black,
semithick,
},
x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\tiny},
y label style={at={(axis description cs:-0.12,.5)},rotate=90,anchor=south,font=\tiny},
x grid style={darkgray176},
xlabel={$\epsilon$},
xmin=2.6, xmax=33.4,
xtick style={color=black},
y grid style={darkgray176},
ylabel={ACC},
ymin=0.459247501575414, ymax=0.720753097064867,
ytick style={color=black}
]
\path [fill=steelblue31119180, fill opacity=0.2]
(axis cs:4,0.495488400714695)
--(axis cs:4,0.471134119552208)
--(axis cs:8,0.573825218559298)
--(axis cs:16,0.69588391704559)
--(axis cs:32,0.700655316445865)
--(axis cs:32,0.708866479088074)
--(axis cs:32,0.708866479088074)
--(axis cs:16,0.706809600753723)
--(axis cs:8,0.5919483533363)
--(axis cs:4,0.495488400714695)
--cycle;

\path [fill=darkorange25512714, fill opacity=0.2]
(axis cs:4,0.671236894707091)
--(axis cs:4,0.663300004137105)
--(axis cs:8,0.667405408960443)
--(axis cs:16,0.64872853153904)
--(axis cs:32,0.67507986339463)
--(axis cs:32,0.68263927242039)
--(axis cs:32,0.68263927242039)
--(axis cs:16,0.65834713773981)
--(axis cs:8,0.683173306510362)
--(axis cs:4,0.671236894707091)
--cycle;

\path [fill=forestgreen4416044, fill opacity=0.2]
(axis cs:4,0.589910447416111)
--(axis cs:4,0.586156691260066)
--(axis cs:8,0.640640635143339)
--(axis cs:16,0.64123331115237)
--(axis cs:32,0.640622497518217)
--(axis cs:32,0.649952449467695)
--(axis cs:32,0.649952449467695)
--(axis cs:16,0.646538678341057)
--(axis cs:8,0.647112376368614)
--(axis cs:4,0.589910447416111)
--cycle;

\addplot [semithick, steelblue31119180]
table {%
4 0.483311260133451
8 0.582886785947799
16 0.701346758899657
32 0.704760897766969
};
\addlegendentry{$\mind=10$}
\addplot [semithick, darkorange25512714]
table {%
4 0.667268449422098
8 0.675289357735403
16 0.653537834639425
32 0.67885956790751
};
\addlegendentry{$\mind=20$}
\addplot [semithick, forestgreen4416044]
table {%
4 0.588033569338089
8 0.643876505755977
16 0.643885994746714
32 0.645287473492956
};
\addlegendentry{$\mind=40$}
\end{axis}

\end{tikzpicture}


==> figures/ablation/min_degree/reddit/gcn_c_small.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=lightgray204
},
scale only axis,
width=2.25cm,
height=2cm,
tick align=outside,
tick pos=left,
title={Reddit},
title style={yshift=-4pt},
xticklabel style={yshift=2pt},
yticklabel style={xshift=2pt},
tick label style={font=\tiny},
legend style={nodes={scale=0.5, transform shape}},
% major tick length=\MajorTickLength,
every tick/.style={
black,
semithick,
},
x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\tiny},
y label style={at={(axis description cs:-0.12,.5)},rotate=90,anchor=south,font=\tiny},
x grid style={darkgray176},
xlabel={$\epsilon$},
xmin=2.6, xmax=33.4,
xtick style={color=black},
y grid style={darkgray176},
ylabel={ACC},
ymin=0.869623642600484, ymax=0.929801077875518,
ytick style={color=black}
]
\path [fill=steelblue31119180, fill opacity=0.2]
(axis cs:4,0.883923445872697)
--(axis cs:4,0.872358980567531)
--(axis cs:8,0.901390855237169)
--(axis cs:16,0.919163365854363)
--(axis cs:32,0.924299536647549)
--(axis cs:32,0.927065739908471)
--(axis cs:32,0.927065739908471)
--(axis cs:16,0.923085705111293)
--(axis cs:8,0.905097125661526)
--(axis cs:4,0.883923445872697)
--cycle;

\path [fill=darkorange25512714, fill opacity=0.2]
(axis cs:4,0.901205130589604)
--(axis cs:4,0.895829140455044)
--(axis cs:8,0.91111645676936)
--(axis cs:16,0.914355992521677)
--(axis cs:32,0.914660708629969)
--(axis cs:32,0.921520466531153)
--(axis cs:32,0.921520466531153)
--(axis cs:16,0.918514768478628)
--(axis cs:8,0.914465648323723)
--(axis cs:4,0.901205130589604)
--cycle;

\path [fill=forestgreen4416044, fill opacity=0.2]
(axis cs:4,0.89878166463381)
--(axis cs:4,0.891121931222786)
--(axis cs:8,0.897491871866255)
--(axis cs:16,0.901811399876718)
--(axis cs:32,0.903877016652382)
--(axis cs:32,0.905792121455081)
--(axis cs:32,0.905792121455081)
--(axis cs:16,0.905337227665784)
--(axis cs:8,0.900781111635531)
--(axis cs:4,0.89878166463381)
--cycle;

\addplot [semithick, steelblue31119180]
table {%
4 0.878141213220114
8 0.903243990449347
16 0.921124535482828
32 0.92568263827801
};
\addlegendentry{$\mind=10$}
\addplot [semithick, darkorange25512714]
table {%
4 0.898517135522324
8 0.912791052546541
16 0.916435380500152
32 0.918090587580561
};
\addlegendentry{$\mind=20$}
\addplot [semithick, forestgreen4416044]
table {%
4 0.894951797928298
8 0.899136491750893
16 0.903574313771251
32 0.904834569053731
};
\addlegendentry{$\mind=40$}
\end{axis}

\end{tikzpicture}

